Probabilistic Neural-symbolic Models for Interpretable Visual Question Answering

We propose a new class of probabilistic neural-symbolic models, that have symbolic functional programs as a latent, stochastic variable. Instantiated in the context of visual question answering, our probabilistic formulation offers two key conceptual advantages over prior neural-symbolic models for VQA. Firstly, the programs generated by our model are more understandable while requiring lesser number of teaching examples. Secondly, we show that one can pose counterfactual scenarios to the model, to probe its beliefs on the programs that could lead to a specified answer given an image. Our results on the CLEVR and SHAPES datasets verify our hypotheses, showing that the model gets better program (and answer) prediction accuracy even in the low data regime, and allows one to probe the coherence and consistency of reasoning performed.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/methods.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:vqabayes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For a standard neural-symbolic NMN approach to question answering
~\citep{Johnson2017}, we are given an input image $\vi$ and
a question $\vx=(x_1,\cdots,x_N)$ as a sequence of words $x_i$ each encoded using a vocabulary $\cal{V}_\vx$, and must produce answers 
$\va$ by planning and executing a series of modular computations ($\vz=(z_1,\cdots,z_N)$) -- \ie~a program of operations ($z_i\in\cal{V}_{\vz}$) to be executed in order to answer the question. %, where each program is represented as a sequence ofsymbols from a vocabulary ($\cal{V}_{\vz}$). \sml{We don't specify what programs these are. Are they GT? Aligned? Unaligned?} 
Note that $\vz$ here is the prefix serialization of the program and programs themselves often have tree-structured topologies. We denote the dataset of $(\vi, \vx, \va)$ triplets as $\mathcal{D}$. Additionally,
we are provided programs $\vz$ for some input questions ($\vx \in \mathcal{S}$), which
specify the notion of grounding desired by an end user. \rama{Our goal is
to provide faithful explanations on unseen questions (along with correct
answers) consistent with the specified grounding.}

We accomplish this by modeling $\vz$ as a
latent variable that underlies both question
and answer generation given an input image. \rama{Intuitively, we expect this will enable us to learn
a more meaningful latent representation for questions, as modeling
uncertainity should help better handle the potentially underspecified
mapping between questions and programs provided by the user.}
As such, 
our model factorizes $p(\vx, \vz, \va| \vi) = p(\vx|\vz) p(\va| \vi, \vz) p(\vz)$ as in the graphical model shown in~\cref{fig:model}, where the
prior $p(\vz)$ is learnt by training a
neural sequence model on valid strings simulated from known syntax.
Conceptually, this factorization captures the notion that many 
differently-worded questions are reducible to identical underlying semantics (captured by a program), making the program space,
in a sense, a compression of the question space. As mentioned in
~\cref{sec:intro} the model also captures the independence of
questions from answers for an image given programs, which is also
an 
intuitive desiderata for interpretable neural-symbolic models\footnote{\rama{This view also matches finding from \citet{Hu2017NMN} who find models linking questions to answer (via attention) operating in low-program supervision regimes often have syntactically poor programs despite leading to correct answers -- i.e.~the program need not be a sufficient statistic anymore to answer the question. }}.
\begin{comment}
It follows naturally then that the linguistics of question generation are 
irrelevant to the answer if the underlying program semantics are known. 
%
Conversely, with this model, we can sample a program, and then infer a
distribution over possible questions (many of which may have surface variations but reduce to the same
underlying semantics). As such, the program space can serve as a lossy encoding for questions, preserving their
``essence'' while ignoring differences in surface forms.
\end{comment}

%In fact, while they may not have realized it, \todo{Devi: I'd drop ``while they may not have realized it,'' -- why try and guess / pass judgment on what other researchers did or did not realize? Should also be careful to not sound like we are modeling the process used to generate some synthetic datasets, and not how VQA should/can be solved in general. We could drop the whole sentence. Or add a footnote ``Interestingly, this is the \emph{the exact generative process} 
%used for curating some synthetic VQA datasets~\citep{CLEVR}''. Also, can we not cite Shapes for this too? The questions must have been generated programmatically. Is there no linguistic variation on the questions?} 
%this model encodes \emph{the exact generative process} 
%used for curating some synthetic VQA datasets 
%that neural module networks have been applied on 
%\citep{CLEVR}. 
%which produce questions to match already generated programs.
%\todo{Deal with the fact that we don't have results on CLEVR.\sml{I would just ignore it here}}

Given the proposed model shown in Figure \ref{fig:model}, we must address two tasks to put the model to use for VQA -- learning model parameters, and performing inference for a specific query.

\noindent\textbf{Learning.} We will always condition on images $\vi$ but may not observe underlying programs $\vz$, so our per-data point training objective is the log-marginal-conditional-likelihood: $\log p(\vx, \va \mid \vi)$. Since computing this
objective involves an intractable summation over latent programs ($\log \sum_\vz p(\vx_j, \vz, \va_j \mid \vi_j)$), we use a variational approximation~\citep{Jordan1999VI}. 
%
Specifically, let \vspace{-4pt}% 
\begin{compactitem}[\hspace{5pt}-]
\item \retwo{$q_\phi(\vz\mid\vx)$ denote an amortized inference neural network parameterized by $\phi$,}\reb{ which instantiates a sequence to sequence LSTM~\citep{Hochreiter1997-xj} model}
\item $p_{\theta_{\vz}}(\va \mid \vz, \vi)$ be a NMN parametrized by $\theta_\vz$ run on image $\vi$ with program $\vz$, 
\item $p_\sigma(\vx \mid \vz)$ be a recurrent network (\reb{sequence to sequence model}) parametrized by $\sigma$ that maps programs to questions, and
\item \retwo{$p(\vz)$ be a prior over programs learned from data or based on program syntax directly \vspace{-2pt}}, \reb{parameterized as an
      LSTM~\citep{Hochreiter1997-xj} sequence model}
\end{compactitem}
%
\rama{Then, for datapoints without program supervision, the objective is:}
\begin{equation*}
\elbo(\va, \vx| \vi) = E_{z \sim q_{\phi}(\vz | \vx)}
[\log p_{\theta_{\vz}}(\va | \vz, \vi) + \log p_{\sigma}(\vx| \vz)] - \beta \KL( q_{\phi}(\vz| \vx), p(\vz))
\end{equation*}
It is easy to show that $\elbo(\vx, \va| \vi) \leq \log p(\vx, \va| \vi)$ for $\beta \ge1$;
as such, maximizing this objective is a form of approximate maximum likelihood training for distribution parameters  $\theta_{\vz}$, $\sigma$, and $\phi$.

Additionally, for data points with annotations, we
add the likelihood of the program given the question
$\log r_\phi(\vz| \vx)$ to the objective. Note that $r$ shares parameters $\phi$ with the inference network $q$. So our overall objective becomes:\\[-8pt]
%
\begin{equation}
\label{eqn:elbo}
\elbo(\va, \vx| \vi) + \alpha \log r(\vz|\vx)\cdot \ind{\vx \in \mathcal{S}}
\end{equation}\\[-4pt]
%
where the indicator function $\ind{\vx\in\mathcal{S}}$ is 1 if $\vx$ is in the supervised set and 0 otherwise and $\alpha$ is a positive scaling factor. The goal is to learn the desired association
of questions with programs from the second term, and to propagate them
to other questions using the first term.

%
%
%
%We are assuming joint model between the question $\vx$ and $\va$, where there is information asymmetry between the
%question and the answer modalities, which might seem a bit confounding at first. Note that for the right model family
%$p$, one would expect that posterior (program) given image and answer $p(\vz| \vi, \va)$ would be more entropic than the
%posterior given questions $p(\vz| \vx)$, thus, we
%can still learn a joint space for variables which have different amounts of information in them. \todo{Not clear what the point here is.\sml{agreed. not sure what the point here is, would remove}}
%
%Exact inference in the model shown in~\cref{fig:model} is intractable in general \sml{say why?} and thus we adopt variational
%inference~\citep{Jordan1999VI}, specifically, amortized inference similar to that used in variational autoencoder
%models~\citep{Kingma2014}. The key difference being that our latent variable is not Gaussian but rather a distribution over a stThructured discrete random variable $\vz$ (\ie programs). Armed with an approximate posterior $q(\vz| \vx)$, we can write the evidence lower
%bound (ELBO), for a single datapoint as
%
%


\noindent\textbf{Inference.} At test time, we can answer questions for images
by computing $p(\va| \vi, \vx) =
\sum_{z} p(\va| \vi, \vz) p(\vz| \vx)$ using an approximation
$p_q(\va| \vi, \vx) \approx E_{\vz_i\sim q(\vz| \vx)} p(\va| \vi, \vz_i)$.

\noindent\textbf{Challenges.} While the $\elbo$ term in~\cref{eqn:elbo} appears similar to a standard ELBO for joint
latent variable models~\citep{Vedantam2018generative,Wang2016,Suzuki2017}, 
there are a few important departures: 
\begin{compactitem}[\hspace{3pt}-]\vspace{-4pt}
\item Firstly, the
latent variable $\vz$ is not a Gaussian or categorical random variable (which admit 
straightforward reparameterizations~\citep{Maddison2017,Jang2016-xb}) 
but rather a sequence of discrete tokens, which complicates the
optimization problem in~\cref{eqn:elbo}.

\item Secondly, the conditional log-likelihood for $\va$ is parameterized by a NMN 
that is dynamically assembled based on sample programs drawn from $q(\vz| \vx)$. 
Depending upon the uncertainty of the
program posterior, program tokens may not be consistently grounded across examples, making learning the appropriate computation for the corresponding neural modules difficult.
%
%and it can be hard to ground a token ${v} \in \cal{V}_{\vz}$ to 
%the ``semantics'' of the operation that the
%module for $v$ is supposed to perform -- \eg~relating the module that we name 
%\texttt{find[red]} to computation 
%that finds red in an input image.

\item Lastly, our observations $\vx$ are explained by powerful ``autoregressive'' sequence models. Learning meaningful latent variable models that are informative of observations for such models is difficult (c.f. ~\citep{Bowman2016,Chen2016_vlae,Alemi2017broken}) as powerful decoder models can explain the data using stochasticity from sampling (referred to
as autodecoding in~\citet{Alemi2017broken}).
Consequently, it also becomes hard to learn meaningful NMN parameters
from the previous step.
\end{compactitem}
In the following sections, we present a training regime and adjustments to the objective in ~\cref{eqn:elbo} that make optimization
more tractable and enable training NMNs with significantly reduced question-aligned program supervision. \rama{While instantiated for question answering, it is not
difficult to conceive versions of this regime for other problems
relevant to probabilistic neural-symbolic models.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Optimizing the ELBO for \vqabayes{}}
\label{sec:elbo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Rather than approaching the joint objective directly, we break ELBO training into three stages: 
\begin{compactenum}[\hspace{3pt}1.]\vspace{-4pt}
\item \textbf{Question coding},
where we learn a latent `code' for questions in the latent space of programs,  
\item  \textbf{Module
training}, where we learn the `execution' of the programs from the first stage of training, 
grounding tokens in programs into the operations they perform on images; and 
\item \retwo{\textbf{Joint training}, where we train both stages jointly given the `warm-starts' 
from the other phases.}
\end{compactenum}\vspace{-4pt}

\noindent\textbf{Question Coding.} 
The goal of this stage is to learn a code for questions in the latent
space of programs -- \ie~ an informative mapping from questions to programs.
\begin{comment}
Learning question-consistent program codes can ease issues with training the NMN by increasing the chance that program symbols will be consistently grounded (\eg always mapping the question text `to the left' to a particular program token).
\end{comment}
Given some set of question-aligned programs, we find this coding process effectively propagates these supervised groundings to unsupervised questions, which enable interpretable explanations / groundings of
queries to explanations of ``what'' the model is doing, which is our
primary goal.

%In the question coding stage, the goal is to learn a code for questions in the latent
%space of programs. If we are successful in having a confident posterior $q(\vz| \vy)$ for a question $\vx$, then it can ease issues
%with training neural module network %parameters, since there is a better chance that symbols will be consistently grounded
%to the appropriate functions/operations that %need to be performed.
During question coding, we drop the $p_{\theta_z}(\va| \vz, \vi)$ term from Eq.~\ref{eqn:elbo}, yielding the objective
%We do question coding, replacing the $\elbo(\va, \vx|\vi)$ term in~\cref{eqn:elbo}
%with a lower bound on the marginal likelihood of questions, making it
%objective:
%
\begin{equation}\label{eqn:elbo_questions}
J(\vx ; \phi, \theta) = E_{z \sim q_{\phi}(\vz | \vx)}
[\log p_{\sigma}(\vx| \vz)] - \beta \KL( q_{\phi}(\vz| \vx), p(\vz))
+ \alpha \log r_{\phi}(\vz| \vx)\cdot \ind{\vx \in \mathcal{S}}
\end{equation}
%
Recent theory from~\citet{Alemi2017broken} prescribes changes
to the ELBO, setting $\beta<1$
as a recipe to learn representations which avoid learning degenerate
latent representations in the presence of powerful decoders.
\reb{Essentially,~\citet{Alemi2017broken} identify that upto a constant factor,
the negative log-marignal likelihood term $D$=$-E_{z \sim q_{\phi}(\vz | \vx)}
[\log p_{\sigma}(\vx| \vz)]$, and the kl diveregence term $R=\KL( q_{\phi}(\vz| \vx), p(\vz))$
bound the mutual information between the data $\vx$ and the latent variable $\vz$ as follows:}
\begin{equation}
	\reb{H - D \leq I(\vx, \vz) \leq R}
\end{equation}
\reb{where $H$ is the entropy of the data, which is a constant. 
One can immediately notice that the standard $\elbo=-D-R$. This means that for the same
value of the $\elbo$ one can get different models which make drastically different usage of the
latent variable (based on the achieved values of $D$ and $R$). Thus, one way to achieve
a desired behavior (of say high mutual information $I(\vx, \vz)$), is to set $\beta$ to a lower
value than the standard $\elbo$ (c.f. Eqn. 6 in~\cite{Alemi2017broken}.)}
This aligns with our goal in question coding, and so we use $\beta<1$.
As this no longer a valid variational lower bound, denote our objective as $J(\vx ; \phi, \theta)$ from now on.

%%%%%%%%%%%%%%%%%%%Comment%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
The ELBO on its own
Moreover,~\cite{Miao2016} note that biasing  $q(\vz|
\vx)$ to contain information about $\vx$ encourages the model to actually utilize the latent space rather than setting the posterior $q_{\sigma}(\vz| \vx)$ to the prior to reduce KL while relying on powerful autoregressive decoders to maintain low loss on question reconstruction -- also known as an \emph{auto-decoding} solution \citep{Alemi2017Broken}.
We do this by setting up the following
semi-supervised learning objective. Given a set of question-aligned programs $\mathcal{S}$, 
we train the variational parameters $\phi$ on both the supervised and unsupervised pairs, writing
%
\begin{equation}
\label{eqn:qn_coding}
J(\vx~;~\phi, \theta)= E_{z \sim q_{\phi}(\vz | \vx)}
\left[\frac{\log p_{\sigma}(\vx| \vz) p(z)^{\beta}}{q_{\phi}(\vz| \vx)^{\beta}}\right] + \alpha \log r_{\phi}(\vz|\vx) \cdot \ind{\vx \in \mathcal{S}}
\label{eqn:qn_coding}
\end{equation}

%
where the indicator function $\ind{\vx\in\mathcal{S}}$ is 1 if $\vx$ is in the supervised set and 0 otherwise, and $r$
denotes a now distribution (different from $p$, $q$). 
\end{comment}

We optimize the above objective using the score function estimator~\citep{Glynn1990}, also referred to as REINFORCE ~\citep{Williams1992} applied to the first term, with a moving average baseline.%\footnote{We experimented with more sophisticated input-dependent baselines~\citep{Miao2016} but did not find them to improve performance in our setting, likely because we use a large, representative batch size of 576. We also tried parameterizing the sequence with the concrete distribution~\citep{Maddison2017,Jang2017}, but it is not clear how to do MLE (second term in~\cref{eqn:qn_coding} with concrete random variables given categorical observations).}
 Finally, while the KL term (in the reward) encourages the
model to generate high-likelihood plausible sequences, we
also penalize the model for producing syntactically invalid programs.


\retwo{Although gradients for the KL term
in~\cref{eqn:elbo_questions} can be computed by decomposing the 
KL for the sequence into per-timestep monte-carlo gradients, we found that 
having one term with per-timestep gradients and another that only receives sequence-level rewards (the
likelihood term) skewed the model towards minimizing the KL, leading to auto-decoding 
solutions. 
Thus, we apply REINFORCE on the entire sequence and 
compute rewards using the full monte carlo gradient,}\reb{\ie{}, we do not optimize the KL term
separately, but instead maximize:}
\begin{equation}\label{eqn:nmn_training_actual}
\reb{E_{\vz\sim q_{\phi}(\vz|\hat{\vx})}\left[\log\left[\frac{ p_{\sigma}(\hat{\vx}| \vz) p(\vz)^{\beta}}{q_{\phi}(\vz| \hat{\vx})^{\beta}}\right]\right]}
\reb{+ \alpha \log r_{\phi}(\hat{\vz}| \hat{\vx})\cdot \ind{\vx \in \mathcal{S}}}
\end{equation}
\reb{where $\hat{\vx}, \hat{\vz}$ are the questions and programs we observe in the dataset.}
%We also find that we need to set $\alpha>1$ for optimization reasons, 
%since otherwise the gradient for $\phi$ from the $q_\phi(\cdot)$ term, 
%which has larger variance and scale dominates the overall gradient signal.

For comparison, the semi-supervised approach in \citet{Johnson2017} can be seen as optimizing the last term on
supervised training data, while our question coding stage optimizes the $\elbo$ in addition to the last term. Our results
in~\cref{sec:results} show that the proposed question coding formulation significantly improves performance relative
to~\citet{Johnson2017} in terms of explaining ``what'' the model is
doing on test programs.

\noindent\textbf{Module Training.}
Having obtained a code for questions in the latent space, we train the parameters of the NMN for question answering. The network modules are trained to perform their corresponding tasks. For example, if the question coding learned to associate the program token $v$ with the question phrase `to the left', then the goal for this second stage is to train the module corresponding to $v$ to actually perform this operation (\eg~\texttt{transform[left]}) when executed on images. 

We do this by optimizing the joint $\elbo(\vx, \va| \vi)$ in \eqref{eqn:elbo} with respect to the parameters $\theta_\vz$ of the neural modules. We write this objective for each instance as
%
\begin{equation}
\label{eqn:nmn_training}
J(\va\mid\vx,\vi;~\theta_\vz) = E_{z\sim q(\vz| \vx)}[\log p_{\theta_z}(\va|\vi, \vz)]
\end{equation}
%
Notably, while we write this objective as a function of
all neural modular network parameters $\theta_\vz$,
for a given instance, only those modules present in the program $
z\sim q(\vz| \vx)$ are updated. In practice, we
take \reb{approx.} argmax decoded programs from $q_{\phi}(\vz|\vx)$ to simplify training, but perform sampling
during joint training in the next stage.
\reb{To be more specific, we run beam search~\citep{Vijayakumar2018} with a beam size of 1 to do this.}
Intuitively, we think
of this as a bias \vs{} variance tradeoff, doing
argmax
enables us to trade off bias for high-variance
from
a posterior which (in the pathological case) could
match
the prior from the first stage of training.
\reb{This is also consistent with standard practice for doing inference in sequence models, where
beam search is the standard inference tool (and sampling often has issues due to teacher forcing
based MLE training, which is how we do semi-supervised learning)~\citep{Bengio2015}.}

%\begin{equation}
%\label{eqn:nmn_training}
%J(\theta_{\mathcal{V}_z}) = E_{\va, \vi, \vx \sim\hat{p}(\va, \vi, \vx)} E_{z\sim q(\vz| \vx)}[\log p_{\theta_z}(\va|\vi, \vz)]
%\end{equation}
%Where $\theta_{\mathcal{V}_\vz}$ is denoting that the parameters for all the
%neural modules $\mathcal{V}_\vz$ are being updated in this step (on expectation
%over the empirical data distribution $\hat{p}(\va, \vi, \vx)$, which places delta
%functions where we observe data).

\noindent\textbf{Joint Training.}
Having trained the question code and the neural module
network parameters, we tune all terms jointly, with the
following objective, which adds scaling factors $\alpha$,
$\beta$ and $\gamma$, and an extra semi-supervised learning term relative to~\cref{eqn:elbo}:
%
\begin{equation}
\label{eqn:final_joint_elbo}
J(\vx, \va|\vi) = E_{z \sim q_{\phi}(\vz | \vx)}
[\gamma \log p_{\theta_{\vz}}(\va | \vz, \vi) + \log p_{\sigma}(\vx| \vz)] - \beta \KL(q_{\phi}(\vz| \vx), p(\vz)) + \alpha \log r_{\phi}(\vz| \vx)
\end{equation}
%
The gamma factor $\gamma$ controls the scaling of the likelihood term for the answers relative to the question (which has more bits of information), similar scaling factors
have been for joint models in~\citet{Vedantam2018generative}. \reb{Similar to~\cref{eqn:nmn_training_actual}, we optimize the full monte
carlo gradient for the above objective as well. The} full training procedure is shown in Algorithm \ref{alg} below.
%\begin{algorithm}
%\small
%\caption{\small \retwo{V-NMN Training}}
%\begin{algorithmic}[1]
%\State Given: $p(\mathbf{z})$, Initialize $q_{\phi}(\mathbf{z}| \mathbf{x})$, $p_{\theta_z}(\mathbf{a}|\mathbf{z}, \mathbf{i})$, $p_{\sigma}(\mathbf{x}|\mathbf{z})$, moving average baseline $B = 0$, $\retwo{\beta=0.1}, \alpha=100.0, \delta=0.99$.
%\State \textbf{Question Coding:} Given $\hat{\vx}, \hat{\vz} \sim p_{data}(\vx, \vz)$, sample $\mathbf{z_i} \sim q_{\phi}(\mathbf{z}| \hat{\vx})$ [\texttt{Repeat until convergence}]
%\Indent
%	\State $\retwo{\nabla_{\phi} \leftarrow (R -B) \log q_{\phi}(\vz_i| \hat{\vx})+ \alpha \nabla_{\phi}\log r_{\phi}(\hat{\vz}| \hat{\vx})}$; where $\retwo{R = \log\left[\frac{ p_{\sigma}(\hat{\vx}| \vz_i) p(\vz_i)^{\beta}}{q_{\phi}(\vz_i| \hat{\vx})^{\beta}}\right]}$
%    \State $\nabla_{\sigma} \leftarrow \nabla_{\sigma} \log p_{\sigma}(\hat{\vx}| \vz_i)$
%    \State $B \leftarrow B + (1 -\delta) (R - B);  \nabla_\theta \leftarrow \nabla_\theta \log p(\hat{\vx} | \vz_i)$
%\EndIndent
%
%\State \textbf{Question Coding:} Given $\hat{\vx}, \hat{\vz} \sim p_{data}(\vx, \vz)$, sample $\mathbf{z_i} \sim q_{\phi}(\mathbf{z}| \hat{\vx})$ [\texttt{Repeat until convergence}]
%\State \textbf{Module Training:} Given $\hat{\vx}, \hat{\va}, \hat{\vi}\sim p_{data}(\vx, \va, \vi)$, $\vz_i=\text{argmax } q(\vz |\hat{\vx})$ [\texttt{Repeat until convergence}]
%\Indent
%    \State $\nabla_{\theta_z} \leftarrow \nabla_{\theta_z} \log p(\hat{\va} | \vz_i, \hat{\vi})$
%\EndIndent
%\State \textbf{Joint Training:} Given $\hat{\vx}, \hat{\va}, \hat{\vi}, \hat{\vz} \sim p_{data}(\vx, \va, \vi, \vz)$, $\vz_i \sim q(\vz| \hat{\vx})$, $\gamma$; Initialize $B = 0$, [\texttt{Repeat until convergence}]
%\Indent
%	\State $\retwo{\nabla_{\phi} \leftarrow (R -B) \nabla_{\phi} \log q_{\phi}(\vz_i| \hat{\vx}) + \alpha \nabla_{\phi}\log r_{\phi}(\hat{\vz}| \hat{\vx})}$; where $\retwo{R = \log\left[\frac{ p_{\sigma}(\hat{\vx}| \vz_i) p(\hat{\va}| \vz_i, \hat{\vi})^\gamma p(\vz_i)^{\beta}}{q_{\phi}(\vz_i| \hat{\vx})^{\beta}}\right]}$
%    \State $B \leftarrow B + (1 -\delta) (R - B);\nabla_\theta \leftarrow \nabla_\theta \log p(\hat{\vx} | \vz_i); \nabla_{\theta_z} \leftarrow \nabla_{\theta_z} \log p(\hat{\va} | \vz_i, \hat{\vi})$
%\EndIndent
%\end{algorithmic}
%\label{alg}
%\end{algorithm}

==> sections/methods_icml.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:vqabayes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As explained in the previous section, our approach embeds a neural-symbolic model for VQA
into a probabilistic graphical model to make them more understandable, by 1) focussing
on making them more legible with less supervision, and 2) more transparent.

In this section we first explain the details of the graphical model, and then provide a
principled training
algorithm based on variational inference~\cite{Jordan1999VI},
and a discussion of how the above desiderata
are addressed by the model.

Let $\vi \in \mathbb{R}^N$ be an input image, 
$\vx$ be a question, which is comprised of a sequence of words
$(x_1, \cdots, x_N)$, where $x_i$ is encoded using a vocabulary $V$ (a set of words),
\ie $x_i \in \{1,\cdots, |V|\}$,
$a \in \{1, \cdots, |A|\}$ be the answer
(where $A$ is the answer vocabulary),
and $\vz$ be the prefix serialization of a program, \ie $\vz = (z_1, \cdots, z_M) \ni z_i \in
\{1, \cdots, |U|\}$, where $U$ is the program vocabulary.
The serialized programs more generally express tree structured, modular computations that
we would like to perform on the image to obtain the answer.
We operate in the semi-supervised setting, assuming access to a limited number of
examples $N$ where all the variables $(\vx, \vz, \vi, a)$ are observed, and a larger
set of examples $M$ where the programs are not observed (\ie are latent).
Our goal is
to provide faithful explanations on unseen questions (along with correct
answers) consistent with the specified grounding, which we accomplish by modeling
$\vz$ explicitly as the latent variable.

This expresses an intuitive independence assumption for \nsym{} VQA models, namely that 
the questions $\vx$ are independent of the answer $a$ given the program $\vz$ ($a \perp \vx\mid\vi$). In other words,
$\vz$ (at inference) is a sufficient statistic for answering the question.
Modeling $\vz$ as a stochastic latent variable helps better handle the uncertainity
in programs for questions in settings where we have a small number of question-program
examples, helping to achieve better legibility with less supervision. Further, with the proposed
model, it becomes easy to pose our high-level transparency desiderata as drawing samples from a
posterior $p(\vz\mid \vi, a)$, where $a$ is a counterfactual answer that can be
specified by a user.

%For a standard neural-symbolic NMN approach to question answering
%~\citep{Johnson2017}, we are given an input image $\vi$ and
%a question $\vx=(x_1,\cdots,x_N)$ as a sequence of words $x_i$ each encoded using a vocabulary $\cal{V}_\vx$, and must produce answers 
%$\va$ by planning and executing a series of modular computations ($\vz=(z_1,\cdots,z_N)$) -- \ie~a program of operations ($z_i\in\cal{V}_{\vz}$) to be executed in order to answer the question. %, where each program is represented as a sequence ofsymbols from a vocabulary ($\cal{V}_{\vz}$). \sml{We don't specify what programs these are. Are they GT? Aligned? Unaligned?} 
%Note that $\vz$ here is the prefix serialization of the program and programs themselves often have tree-structured topologies. We denote the dataset of $(\vi, \vx, \va)$ triplets as $\mathcal{D}$. Additionally,
%we are provided programs $\vz$ for some input questions ($\vx \in \mathcal{S}$), which
%specify the notion of grounding desired by an end user. \rama{Our goal is
%to provide faithful explanations on unseen questions (along with correct
%answers) consistent with the specified grounding.}

%We accomplish this by modeling $\vz$ as a
%latent variable that underlies both question
%and answer generation given an input image. \rama{Intuitively, we expect this will enable us to learn
%a more meaningful latent representation for questions, as modeling
% by the user.}
%As such, 
%our model factorizes $p(\vx, \vz, \va\mid \vi) = p(\vx\mid\vz) p(\va\mid \vi, \vz) p(\vz)$ as in the graphical model shown in~\cref{fig:model}, where the
%prior $p(\vz)$ is learnt by training a
%neural sequence model on valid strings simulated from known syntax.
%Conceptually, this factorization captures the notion that many 
%differently-worded questions are reducible to identical underlying semantics (captured by a program), making the program space,
%in a sense, a compression of the question space. As mentioned in
%~\cref{sec:intro} the model also captures the independence of
%questions from answers for an image given programs, which is also
%an 
%intuitive desiderata for interpretable neural-symbolic models }}.

%In fact, while they may not have realized it, \todo{Devi: I'd drop ``while they may not have realized it,'' -- why try and guess / pass judgment on what other researchers did or did not realize? Should also be careful to not sound like we are modeling the process used to generate some synthetic datasets, and not how VQA should/can be solved in general. We could drop the whole sentence. Or add a footnote ``Interestingly, this is the \emph{the exact generative process} 
%used for curating some synthetic VQA datasets~\citep{CLEVR}''. Also, can we not cite Shapes for this too? The questions must have been generated programmatically. Is there no linguistic variation on the questions?} 
%this model encodes \emph{the exact generative process} 
%used for curating some synthetic VQA datasets 
%that neural module networks have been applied on 
%\citep{CLEVR}. 
%which produce questions to match already generated programs.
%\todo{Deal with the fact that we don't have results on CLEVR.\sml{I would just ignore it here}}

Next, we explain how we parameterize the model, and then derive an
algorithm for semi-supervised learning with such a model.

\subsection{Parameterization} We parameterize the terms in the above graphical model using neural networks. Firstly,
the prior over programs $p(\vz)$ is parameterized using an LSTM~\citep{Hochreiter1997-xj} sequence model, and pretrained
using maximum likelihood, either on programs simulated using the syntax of the program (unless specified otherwise). The
prior is learned first and kept fixed for the rest of the training process. Next, $p_\sigma(\vx \mid \vz)$
is an LSTM sequence to sequence model~\citep{Sutskever2014} parametrized by $\sigma$ that maps programs to questions.
Likewise, $q_\phi(\vz \mid \vx)$ is an LSTM sequence to sequence model that maps questions to programs.
Finally, $p(a\mid\vz, \vi)$ is a neural-symbolic model, which assembles a neural network based on the symbolic
functional program (on the fly) and predicts an answer\todo{make a reference to the initial figure}. 
Each symbol $u \in U$, the program vocabulary has an associated neural network parameterized
by $\theta_u$. The mapping $p(a\mid\vz, \vi)$ then is operationalized as
$p_{\theta_z}(a\mid\vi)$, where $\theta_\vz = \{ \theta_u : u \in \vz\}$.
For reference, previous neural-symbolic models for VQA~\cite{Hu2017NMN,Johnson2017,Mascharka2018}
model $q_\phi(\vz \mid \vx)$ and $p_{\theta_{\vz}(\va \mid \vz, \vi)}$ terms from our present model.

\subsection{Learning}
For the $M$ examples where we do not observe any programs, our log-evidence is:
$\log p(\vx, a| \vi)$. Since computing this
objective involves an intractable summation over latent
programs ($\log \sum_\vz p(\vx, \vz, \va \mid \vi)$),
we use a variational approximation~\citep{Jordan1999VI} -- choosing
an amortized inference network $q_\phi(\vz|\vx)$:
\begin{multline}
    \elbo(\va, \vx| \vi) = E_{z \sim q_{\phi}(\vz | \vx)}
    [\log p_{\theta_{\vz}}(\va | \vi) + \log p_{\sigma}(\vx| \vz)] \\
    - \beta \KL( q_{\phi}(\vz| \vx), p(\vz))
\end{multline}

It is easy to show that $\elbo(\vx, \va| \vi) \leq \log p(\vx, \va| \vi)$ for $\beta \ge1$;
as such, maximizing this objective is a form of approximate maximum likelihood training
for distribution parameters  $\theta_{\vz}$, $\sigma$, and $\phi$.
Additionally, for the $N$ data points with program annotations, we
add the likelihood of the program given the question
$\log q_\phi(\vz| \vx)$ to the objective, in order to capture
the associations between the question and program spaces:

\begin{equation}
\label{eqn:elbo}
\sum_M \elbo(\va, \vx| \vi) + \alpha \sum_N \log q_{\phi}(\vz|\vx)
\end{equation}\\[-4pt]
where, $\alpha > 0$ is a scalar. 
The goal is to learn the desired association
of questions with programs from the second term, and to propagate them
to other questions using the first term.

Two issues complicate the optimization of~\cref{eqn:elbo} in the
setting where $N << M$, which is of interest for data-efficient
legibility: firstly,
inference in the exponential space of possible programs is difficult, and
unlike gaussian or categorical posteriors does not admit straightforward
reparameterization to reduce variance, and
secondly, one has to learn how to execute the programs, which is challenging,
since the optimization landscape for $p(a|\vz, \vi)$ is discontinuous
in the space of programs. This adds noise to the gradients
$\nabla \log q_{\phi}(\vz|\vx)$ making credit assignment difficult.

Rather than approaching objective~\cref{eqn:elbo} directly, our key insight
is to break the training into three stages:
\begin{compactenum}[\hspace{3pt}1.]\vspace{-4pt}
\item \textbf{Question Coding},
where we learn a latent `code' for questions in the latent space of programs,  
\item  \textbf{Module
training}, where we learn the `execution' of the programs from the first stage of training, 
grounding tokens in programs into the operations they perform on images; and 
\item \retwo{\textbf{Joint training}, where we train both stages jointly given the `warm-starts' 
from the other phases.}
\end{compactenum}\vspace{-4pt}

\noindent\textbf{Question Coding.} 
The goal of this stage is to learn a code for questions in the latent
space of programs -- \ie~ an informative mapping from questions to programs.
Given some set of question-aligned programs, we find this coding process effectively propagates these supervised groundings to unsupervised questions, which enable interpretable explanations / groundings of
queries to explanations of ``what'' the model is doing, which is our
primary goal.

In this stage, instead of dealing with the complexity of the $p_{\theta_z}(\va|\vi)$
mapping, we instead work with the evidence $p(\vx) = \sum_a p(a, \vx|\vi)$.
Doing this, similar to~\cref{eqn:elbo} we get the following objective:

%In the question coding stage, the goal is to learn a code for questions in the latent
%space of programs. If we are successful in having a confident posterior $q(\vz| \vy)$ for a question $\vx$, then it can ease issues
%with training neural module network %parameters, since there is a better chance that symbols will be consistently grounded
%to the appropriate functions/operations that %need to be performed.
%During question coding, we drop the $p_{\theta_z}(\va| \vz, \vi)$ term from Eq.~\ref{eqn:elbo}, yielding the objective
%We do question coding, replacing the $\elbo(\va, \vx|\vi)$ term in~\cref{eqn:elbo}
%with a lower bound on the marginal likelihood of questions, making it
%objective:
%
\begin{multline}
\label{eqn:elbo_questions}
J(\vx ; \phi, \sigma) = E_{z \sim q_{\phi}(\vz | \vx)}
[\log p_{\sigma}(\vx| \vz)] - \\\beta\cdot\KL( q_{\phi}(\vz| \vx), p(\vz))
+ \alpha \log r_{\phi}(\vz| \vx)\cdot \ind{\vx \in \mathcal{S}}
\end{multline}
Note that 

Conceptually, our question coding objective is
similar to prior work~\citep{Yin2018,Miao2016},
which also work with discrete, sequential latent spaces and set values of
$\beta<1$ and scale the contribution of $\alpha$ relative to the $\elbo$.
Beyond empirical justifications,
recent results from~\citet{Alemi2017Broken} provide further
insight for why $0<\beta<1$ is a useful setting to learn meaningful latent
variable models with high mutual information $I(\vx, \vz)$, which is challenging when
when the $\vx$ decoder makes no conditional independence assumptions
(which is the case when decoding questions with an LSTM). We provide
a more detailed summary
a summary of their results in the supplementary material.

As this no longer a valid variational lower bound, we
denote our objective as $J(\vx ; \phi, \sigma)$ from now on.

\begin{equation}\label{eqn:nmn_training_actual}
\reb{E_{\vz\sim q_{\phi}(\vz|\hat{\vx})}\left[\log\left[\frac{ p_{\sigma}(\hat{\vx}| \vz) p(\vz)^{\beta}}{q_{\phi}(\vz| \hat{\vx})^{\beta}}\right]\right]}
\reb{+ \alpha \log r_{\phi}(\hat{\vz}| \hat{\vx})\cdot \ind{\vx \in \mathcal{S}}}
\end{equation}
We optimize the above objective using the score function
estimator~\citep{Glynn1990}, also referred to as
REINFORCE~\citep{Williams1992} applied to the first term, with a moving
average baseline.%\footnote{We experimented with more sophisticated input-dependent baselines~\citep{Miao2016} but did not find them to improve performance in our setting, likely because we use a large, representative batch size of 576. We also tried parameterizing the sequence with the concrete distribution~\citep{Maddison2017,Jang2017}, but it is not clear how to do MLE (second term in~\cref{eqn:qn_coding} with concrete random variables given categorical observations).}
Finally, while the KL term (in the reward) encourages the
model to generate high-likelihood plausible sequences, we
also penalize the model for producing syntactically invalid programs.

\retwo{Although gradients for the KL term
in~\cref{eqn:elbo_questions} can be computed by decomposing the 
KL for the sequence into per-timestep monte-carlo gradients, we found that 
having one term with per-timestep gradients and another that only receives sequence-level rewards (the
likelihood term) skewed the model towards minimizing the KL, leading to auto-decoding 
solutions. 
Thus, we apply REINFORCE on the entire sequence and 
compute rewards using the full monte carlo gradient,}\reb{\ie{}, we do not optimize the KL term
separately, but instead maximize:}

\reb{where $\hat{\vx}, \hat{\vz}$ are the questions and programs we observe in the dataset.}

For comparison, the semi-supervised approach in \citet{Johnson2017} can be seen as optimizing the last term on
supervised training data, while our question coding stage optimizes the $\elbo$ in addition to the last term. Our results
in~\cref{sec:results} show that the proposed question coding formulation significantly improves performance relative
to~\citet{Johnson2017} in terms of explaining ``what'' the model is
doing on test programs.


%$\theta_\vz$
%space is 
%is highly structured and discrete, which makes inference (in the exponential)
%space of programs hard.
%
%While the $\elbo$ term in~\cref{eqn:elbo} appears similar to a standard ELBO for joint
%latent variable models~\citep{Vedantam2018generative,Wang2016,Suzuki2017}, 
%there are a few important departures: 
%\begin{compactitem}[\hspace{3pt}-]\vspace{-4pt}
%\item Firstly, the
%latent variable $\vz$ is not a Gaussian or categorical random variable (which admit 
%straightforward reparameterizations~\citep{Maddison2017,Jang2016-xb}) 
%but rather a sequence of discrete tokens, which complicates the
%optimization problem in~\cref{eqn:elbo}.
%
%\item Secondly, the conditional log-likelihood for $\va$ is parameterized by a NMN 
%that is dynamically assembled based on sample programs drawn from $q(\vz| \vx)$. 
%Depending upon the uncertainty of the
%program posterior, program tokens may not be consistently grounded across examples,
%making learning the appropriate computation for the
%corresponding neural modules difficult.
%%
%%and it can be hard to ground a token ${v} \in \cal{V}_{\vz}$ to 
%%the ``semantics'' of the operation that the
%%module for $v$ is supposed to perform -- \eg~relating the module that we name 
%%\texttt{find[red]} to computation 
%%that finds red in an input image.
%
%%\item Lastly, our observations $\vx$ are explained by powerful ``autoregressive'' sequence models. Learning meaningful latent variable models that are informative of observations for such models is difficult (c.f. ~\citep{Bowman2016,Chen2016_vlae,Alemi2017broken}) as powerful decoder models can explain the data using stochasticity from sampling (referred to
%%as autodecoding in~\citet{Alemi2017broken}).
%%Consequently, it also becomes hard to learn meaningful NMN parameters
%%from the previous step.
%\end{compactitem}

